Vision-based Underwater Formation Control With Input Saturations via Barrier Lyapunov Functions

In this work, we propose a communication-free framework for vision-based formation control of fully actuated underwater robots subject to sensing constraints, collision-avoidance requirements, and input saturations. Recentered barrier Lyapunov functions encode sensing and collision-avoidance constraints, while command-filtered backstepping extends the design to the second-order vehicle dynamics. The resulting control objective is enforced through a quadratic program that explicitly accounts for actuator limits. Conservative sensing domains provide margins from the physical limits and are adaptively relaxed when necessary, allowing temporary violation of the conservative bounds. The proposed approach is validated through realistic Software-in-the-Loop (SITL) simulations in Gazebo.

==> Sections/stability_analysis.tex <==
This section establishes the main closed-loop properties of the proposed
controller. The analysis is separated into three parts. First, we establish
forward invariance of the physical collision-avoidance and sensing
constraints through the auxiliary domain-enlargement dynamics. Second, we
derive an input-to-state stability estimate for the physical
command-filtered CLF dynamics, where actuator-induced CLF relaxation,
external disturbances, and parent motion enter explicitly as perturbations.
Finally, the directed-tree structure is exploited to obtain a network-level
stability result.

\subsection{Preliminaries and assumptions}

For every follower \(i\in\vertices\setminus\{1\}\), let
\(j\in\neigh_i\) denote its unique parent. Define
\[
    \vect{s}_i
    \define
    \col_{\ell\in\mathcal L}(s_{\ell,i}),
    \qquad
    \vect{v}_i
    \define
    \dot{\vect{s}}_i,
\]
and let \(V_i^{a}\) denote the adaptive composite potential. For the leader, \(V_1\) is the
tracking potential defined in \eqref{eq:leader_tracking_potential}.

We make the following standard assumptions.

\begin{assumption}
\label{ass:closed_loop_analysis}
For every agent \(i\):
\begin{enumerate}
    \item
    \(\inertiaM_i=\inertiaM_i^\top\succ0\) is constant and the marine
    dynamics satisfy
    \[
        \veltwist_i^\top
        \coriolis_i(\veltwist_i)\veltwist_i
        =
        0.
    \]
    The restoring wrench is bounded and the damping is dissipative.

    \item
    The disturbance \(\vect d_i\) is bounded.

    \item
    The desired configuration lies strictly inside the guarded adaptive
    domain, i.e.,
    \[
        h_{\ell,ij}^{d,c}>m_\ell,
        \qquad
        \ell\in\mathcal L.
    \]

    \item
    The auxiliary problem \eqref{eq:adaptive_domain_controller} remains
    feasible along the considered trajectory.

    \item
    The desired formation is dynamically admissible and the hard CLF
    inequality is feasible in a neighborhood of the desired formation set.
\end{enumerate}
\end{assumption}

The last condition is necessarily local in the presence of bounded
actuation: sufficiently far from the desired configuration, the requested
CLF decrease may exceed the available control authority.

\subsection{Forward invariance of the physical constraints}

For every adaptive channel define
\begin{equation}
    \mathcal S_{\ell,ij}
    \define
    \left\{
        (\pose_i,\pose_j,s_{\ell,i}):
        h_{\ell,ij}^{a}\geq m_\ell,\;
        s_{\ell,i}\in[0,1]
    \right\}.
    \label{eq:guarded_adaptive_set}
\end{equation}

\begin{proposition}
\label{prop:adaptive_physical_invariance}
Suppose that
\(
(\pose_i(0),\pose_j(0),s_{\ell,i}(0))
\in\mathcal S_{\ell,ij}
\)
and that the auxiliary controller
\eqref{eq:adaptive_domain_controller} remains feasible. Then
\[
    h_{\ell,ij}^{a}(t)\geq m_\ell,
    \qquad
    s_{\ell,i}(t)\in[0,1],
    \qquad
    \forall t\geq0.
\]
Moreover, the corresponding physical constraint remains strictly satisfied.
\end{proposition}

\begin{proof}
The auxiliary controller satisfies
\[
    \dot h_{\ell,ij}^{a}
    +
    \gamma_\ell
    \left(
        h_{\ell,ij}^{a}-m_\ell
    \right)
    \geq0,
\]
while
\(
v_{\ell,i}\in T_{[0,1]}(s_{\ell,i})
\).
The comparison lemma and Nagumo's theorem therefore imply forward invariance
of \(\mathcal S_{\ell,ij}\).

Let \(h_{\ell,ij}^{p}\) denote the corresponding physical constraint
function. By construction,
\begin{equation}
    h_{\ell,ij}^{p}
    =
    h_{\ell,ij}^{c}
    +
    \bar\rho_\ell
    =
    h_{\ell,ij}^{a}
    +
    \bar\rho_\ell
    \left(
        1-s_{\ell,i}
    \right).
    \label{eq:physical_adaptive_relation}
\end{equation}
Since \(s_{\ell,i}\leq1\),
\[
    h_{\ell,ij}^{p}
    \geq
    h_{\ell,ij}^{a}
    \geq
    m_\ell
    >
    0,
\]
which proves satisfaction of the physical constraint.
\end{proof}

Together with Proposition~\ref{prop:positive_camera_depth},
Proposition~\ref{prop:adaptive_physical_invariance} guarantees preservation
of the complete physical sensing domain.

\subsection{Properties of the adaptive potential}

The positive margin in Proposition~\ref{prop:adaptive_physical_invariance}
also prevents the logarithmic barriers from approaching their singularities.
This provides useful regularity properties for the subsequent stability
analysis.

\begin{lemma}
\label{lem:adaptive_potential_bounds}
Consider any compact subset of the guarded adaptive domain defined by
\[
    h_{\ell,ij}^{a}\geq m_\ell,
    \qquad
    s_{\ell,i}\in[0,1].
\]
Then there exist finite constants
\(c_{\zeta,i}>0\),
\(c_{p,i}>0\), and
\(c_{s,\ell,i}>0\) such that
\begin{subequations}
\label{eq:potential_regular_bounds}
\begin{align}
    \norm{\vect{\zeta}_i}^{2}
    &\leq
    c_{\zeta,i} V_i^{a},
    \\
    \norm{\nabla_{\pos_j}V_i^{a}}^{2}
    &\leq
    c_{p,i} V_i^{a},
    \\
    -
    \frac{\partial V_i^{a}}
         {\partial s_{\ell,i}}
    &\leq
    c_{s,\ell,i}V_i^{a}.
\end{align}
\end{subequations}
\end{lemma}

\begin{proof}
Under Proposition~\ref{prop:adaptive_physical_invariance}, every logarithmic
argument is uniformly separated from zero. Moreover, the physical range
constraint bounds the relative position, while
Proposition~\ref{prop:positive_camera_depth} bounds the camera depth away
from zero. Hence \(V_i^{a}\) and its configuration derivatives are smooth on
the considered compact set.

At the desired formation, \(V_i^{a}\) and all its configuration gradients
vanish. The recentered barriers have quadratic behavior around their desired
values, and the quadratic formation and image-centering terms have the same
property. The first two inequalities therefore follow locally from Taylor
expansion and extend to the compact set by continuity.

Finally, from \eqref{eq:adaptive_barrier_enlargement_derivative},
\[
    -
    \frac{\partial
        \recenteredBarrier_{\ell,ij}^{a}}
        {\partial s_{\ell,i}}
    =
    \bar\rho_\ell
    \frac{
        \left(
            h_{\ell,ij}^{a}
            -
            h_{\ell,ij}^{d,a}
        \right)^2
    }{
        h_{\ell,ij}^{a}
        \left(
            h_{\ell,ij}^{d,a}
        \right)^2
    }.
\]
Both this quantity and
\(\recenteredBarrier_{\ell,ij}^{a}\) vanish quadratically at the desired
constraint value, while their ratio remains bounded on the guarded compact
set. This proves the third inequality.
\end{proof}

The following consequence characterizes the effect of the adaptive dynamics
on the physical CLF.

\begin{lemma}
\label{lem:adaptive_clf_coupling}
Define
\begin{equation}
    \psi_{s,i}
    \define
    \sum_{\ell\in\mathcal L}
    \frac{\partial V_i^{a}}
         {\partial s_{\ell,i}}
    v_{\ell,i}.
    \label{eq:adaptive_clf_coupling}
\end{equation}
Then domain enlargement cannot increase the adaptive potential. Moreover,
there exists \(\kappa_{s,i}\geq0\) such that
\begin{equation}
    \psi_{s,i}
    \leq
    \kappa_{s,i}W_i,
    \qquad
    \kappa_{s,i}
    \define
    \sum_{\ell\in\mathcal L}
    c_{s,\ell,i}k_{s,\ell}.
    \label{eq:adaptive_clf_coupling_bound}
\end{equation}
\end{lemma}

\begin{proof}
From \eqref{eq:adaptive_barrier_enlargement_derivative},
\(
\partial V_i^{a}/\partial s_{\ell,i}\leq0
\).
Consequently, every channel satisfying \(v_{\ell,i}\geq0\) contributes a
nonpositive term to \(\psi_{s,i}\).

The auxiliary controller is the projection of
\(
-k_{s,\ell}s_{\ell,i}
\)
onto a feasible set whose lower boundary can only increase the selected
input. Hence
\[
    v_{\ell,i}
    \geq
    -k_{s,\ell}s_{\ell,i},
\]
and therefore
\[
    \max\{-v_{\ell,i},0\}
    \leq
    k_{s,\ell}s_{\ell,i}
    \leq
    k_{s,\ell}.
\]
Using Lemma~\ref{lem:adaptive_potential_bounds} and
\(V_i^{a}\leq W_i\) gives \eqref{eq:adaptive_clf_coupling_bound}.
\end{proof}

\subsection{Physical CLF estimate}

Recall that the CLF-QP is constructed by freezing the adaptive state and
enforces
\begin{equation}
    a_i
    +
    \vect b_i^\top\vect f_i^\star
    \leq
    -\gamma_i W_i
    +
    \delta_i^\star.
    \label{eq:physical_clf_qp_inequality}
\end{equation}
The complete derivative additionally contains the parent-motion,
disturbance, and adaptive-domain terms. Hence,
\begin{equation}
    \dot W_i
    \leq
    -\gamma_iW_i
    +
    \delta_i^\star
    +
    \chi_i
    +
    \vect e_{\veltwist,i}^{\top}\vect d_i
    +
    \psi_{s,i}.
    \label{eq:complete_physical_clf_inequality}
\end{equation}

For each follower, Lemma~\ref{lem:adaptive_potential_bounds} yields
\begin{equation}
    |\chi_i|
    \leq
    \sqrt{c_{p,i}W_i}\,
    \norm{\veltwist_j}.
    \label{eq:parent_interconnection_bound}
\end{equation}
Moreover,
\[
    \norm{\vect e_{\veltwist,i}}^2
    \leq
    \frac{2}{\lambda_{\min}(\inertiaM_i)}
    W_i.
\]
Applying Young's inequality to
\eqref{eq:parent_interconnection_bound} and to the disturbance term gives,
for arbitrary \(\epsilon_{p,i},\epsilon_{d,i}>0\),
\begin{align}
    \dot W_i
    \leq\;&
    -\lambda_{W,i}W_i
    +
    \delta_i^\star
    +
    \beta_{p,i}
    \norm{\veltwist_j}^{2}
    +
    \beta_{d,i}
    \norm{\vect d_i}^{2},
    \label{eq:local_clf_iss_bound}
    \\
    \lambda_{W,i}
    \define\;&
    \gamma_i
    -
    \kappa_{s,i}
    -
    \epsilon_{p,i}
    -
    \epsilon_{d,i},
    \nonumber
\end{align}
where
\begin{equation}
    \beta_{p,i}
    \define
    \frac{c_{p,i}}{4\epsilon_{p,i}},
    \qquad
    \beta_{d,i}
    \define
    \frac{1}{
        2\epsilon_{d,i}
        \lambda_{\min}(\inertiaM_i)
    }.
    \label{eq:clf_iss_constants}
\end{equation}
For the leader, the parent term is absent and
\(\kappa_{s,1}=0\).

Condition
\begin{equation}
    \gamma_i
    >
    \kappa_{s,i}
    +
    \epsilon_{p,i}
    +
    \epsilon_{d,i}
    \label{eq:clf_decay_gain_condition}
\end{equation}
therefore guarantees a strict ISS-type decay estimate for the physical CLF.

\subsection{Command-filter dynamics}

Unlike command-filtered backstepping schemes in which the filter derivative
is only an approximation of the derivative of the virtual input,
\(\dot{\veltwist}_{i,c}\) is explicitly included in
\eqref{eq:clf_nominal_drift}. The physical CLF inequality therefore holds
for the actual command-filter dynamics and does not require a
singular-perturbation approximation.

To include the filter state explicitly in the stability estimate, define
\begin{equation}
    \widetilde{\veltwist}_{i,c}
    \define
    \veltwist_{i,c}
    -
    \veltwist_{i,\mathrm{ff}},
    \qquad
    F_i
    \define
    \frac{1}{2}
    \norm{\widetilde{\veltwist}_{i,c}}^2.
    \label{eq:filter_storage}
\end{equation}
From \eqref{eq:desired_generalized_velocity} and
\eqref{eq:generalized_velocity_command_filter},
\begin{equation}
    \dot{\widetilde{\veltwist}}_{i,c}
    =
    -
    \matr{\Lambda}_i
    \widetilde{\veltwist}_{i,c}
    -
    \matr{\Lambda}_i
    \matr K_{\eta,i}
    \vect\zeta_i
    -
    \dot{\veltwist}_{i,\mathrm{ff}}.
    \label{eq:filtered_velocity_error_dynamics}
\end{equation}
Using Lemma~\ref{lem:adaptive_potential_bounds} and Young's inequality, there
exist positive constants
\(\lambda_{F,i}\),
\(c_{F,i}\), and
\(c_{\mathrm{ff},i}\) such that
\begin{equation}
    \dot F_i
    \leq
    -
    \lambda_{F,i}F_i
    +
    c_{F,i}W_i
    +
    c_{\mathrm{ff},i}
    \norm{
        \dot{\veltwist}_{i,\mathrm{ff}}
    }^2.
    \label{eq:filter_iss_bound}
\end{equation}

Define the augmented storage function
\begin{equation}
    U_i
    \define
    W_i
    +
    \varepsilon_iF_i,
    \qquad
    \varepsilon_i>0.
    \label{eq:agent_storage_function}
\end{equation}
Choosing \(\varepsilon_i\) sufficiently small so that
\[
    \lambda_{W,i}
    -
    \varepsilon_i c_{F,i}
    >
    0
\]
gives constants
\(\lambda_i>0\),
\(c_{\nu,i}>0\), and
\(c_{r,i}>0\) such that
\begin{equation}
    \dot U_i
    \leq
    -
    \lambda_iU_i
    +
    \beta_{p,i}
    \norm{\veltwist_j}^{2}
    +
    \delta_i^\star
    +
    \beta_{d,i}
    \norm{\vect d_i}^{2}
    +
    c_{r,i}
    \norm{
        \dot{\veltwist}_{i,\mathrm{ff}}
    }^{2},
    \label{eq:agent_iss_storage}
\end{equation}
with the parent term omitted for \(i=1\). Furthermore,
\begin{equation}
    \norm{
        \veltwist_i
        -
        \veltwist_{i,\mathrm{ff}}
    }^{2}
    \leq
    c_{\nu,i}U_i.
    \label{eq:velocity_storage_bound}
\end{equation}

\subsection{Directed-tree interconnection}

We now exploit the directed-tree structure. Number the agents according to
their depth from the leader so that the parent of every follower has a lower
index. For a stationary formation objective,
\(
\veltwist_{i,\mathrm{ff}}=\boldsymbol 0
\)
for the followers and the leader reference eventually satisfies
\(
\veltwist_{1,\mathrm{ff}}=\boldsymbol 0
\).
Using \eqref{eq:velocity_storage_bound} for the parent of each follower,
\eqref{eq:agent_iss_storage} becomes
\begin{equation}
    \dot U_i
    \leq
    -
    \lambda_iU_i
    +
    \kappa_{ij}U_j
    +
    q_i,
    \qquad
    j\in\neigh_i,
    \label{eq:tree_agent_comparison}
\end{equation}
where
\begin{equation}
    \kappa_{ij}
    \define
    \beta_{p,i}c_{\nu,j},
    \qquad
    q_i
    \define
    \delta_i^\star
    +
    \beta_{d,i}
    \norm{\vect d_i}^{2}.
    \label{eq:agent_perturbation}
\end{equation}
For the leader,
\[
    \dot U_1
    \leq
    -
    \lambda_1U_1
    +
    q_1.
\]

Collecting
\(
\vect U=\col(U_1,\ldots,U_N)
\)
and
\(
\vect q=\col(q_1,\ldots,q_N)
\),
the comparison system takes the form
\begin{equation}
    \dot{\vect U}
    \leq
    \matr A_U\vect U
    +
    \vect q,
    \label{eq:network_comparison_system}
\end{equation}
where \(\matr A_U\) has diagonal entries
\(-\lambda_i\) and, for every follower \(i\) with parent \(j\),
the entry
\(
[\matr A_U]_{ij}=\kappa_{ij}
\);
all other off-diagonal entries are zero.

Under the above topological ordering,
\(\matr A_U\) is lower triangular with strictly negative diagonal entries.
It is therefore Hurwitz and Metzler.

\begin{theorem}
\label{thm:closed_loop_practical_stability}
Consider the closed-loop system under
Assumption~\ref{ass:closed_loop_analysis}. Suppose that
\eqref{eq:clf_decay_gain_condition} holds and that the trajectory remains in
the guarded region in which Lemma~\ref{lem:adaptive_potential_bounds}
applies. Then:

\begin{enumerate}
    \item
    the physical collision-avoidance and sensing constraints are forward
    invariant;

    \item
    the directed-tree formation dynamics satisfy the comparison estimate
    \begin{equation}
        \vect U(t)
        \leq
        e^{\matr A_U(t-t_0)}
        \vect U(t_0)
        +
        \int_{t_0}^{t}
        e^{\matr A_U(t-\tau)}
        \vect q(\tau)
        \,d\tau;
        \label{eq:network_iss_estimate}
    \end{equation}

    \item
    if \(\vect q\in\mathcal L_\infty\), the formation errors, generalized
    velocity errors, and command-filter states are ultimately bounded;

    \item
    if
    \(
    \vect q(t)\rightarrow\boldsymbol 0
    \),
    then
    \(
    \vect U(t)\rightarrow\boldsymbol 0
    \).
\end{enumerate}
\end{theorem}

\begin{proof}
The first statement follows from
Proposition~\ref{prop:adaptive_physical_invariance}.
The differential inequalities
\eqref{eq:tree_agent_comparison} yield
\eqref{eq:network_comparison_system}. Since
\(\matr A_U\) is Metzler, the comparison principle gives
\eqref{eq:network_iss_estimate}. Since \(\matr A_U\) is also Hurwitz, bounded
\(\vect q\) implies bounded \(\vect U\), whereas
\(
\vect q(t)\rightarrow\boldsymbol0
\)
implies
\(
\vect U(t)\rightarrow\boldsymbol0
\).
The result then follows from
\eqref{eq:agent_storage_function} and
\eqref{eq:velocity_storage_bound}.
\end{proof}

For a constant bound
\(
0\leq\vect q(t)\leq\overline{\vect q}
\),
Theorem~\ref{thm:closed_loop_practical_stability} additionally yields the
componentwise ultimate estimate
\begin{equation}
    \limsup_{t\rightarrow\infty}
    \vect U(t)
    \leq
    -
    \matr A_U^{-1}
    \overline{\vect q}.
    \label{eq:network_ultimate_bound}
\end{equation}
Thus, the CLF-QP relaxation has a direct interpretation as a measure of the
performance degradation induced by the available control authority.

\subsection{Nominal convergence and recovery of the conservative domain}

The previous result treats
\(\delta_i^\star\) as an explicit actuation-deficit signal. We now consider
the nominal regime in which the desired CLF decrease becomes compatible with
the available control authority.

\begin{corollary}
\label{cor:nominal_convergence}
Suppose that the assumptions of
Theorem~\ref{thm:closed_loop_practical_stability} hold, that the desired
leader reference is stationary, and that
\[
    \vect d_i(t)\rightarrow\boldsymbol0,
    \qquad
    \delta_i^\star(t)\rightarrow0,
    \qquad
    \forall i\in\vertices.
\]
Then
\[
    U_i(t)\rightarrow0,
    \qquad
    \forall i\in\vertices.
\]
Consequently, the formation converges to the zero set of the composite
potential and
\[
    \vect e_{\veltwist,i}\rightarrow\boldsymbol0,
    \qquad
    \veltwist_i\rightarrow\boldsymbol0.
\]
Moreover,
\[
    s_{\ell,i}(t)\rightarrow0,
    \qquad
    \ell\in\mathcal L,
\]
so that the nominal conservative domains are asymptotically recovered.
\end{corollary}

\begin{proof}
The first statement follows immediately from
Theorem~\ref{thm:closed_loop_practical_stability} because
\(\vect q(t)\rightarrow\boldsymbol0\).
Thus
\(
W_i\rightarrow0
\)
and
\(
F_i\rightarrow0
\).
By positive definiteness of the corresponding terms,
the configuration converges to the zero set of \(V_i^a\), while
\(
\vect e_{\veltwist,i}\rightarrow0
\)
and
\(
\widetilde{\veltwist}_{i,c}\rightarrow0
\).

At the desired configuration,
\(
h_{\ell,ij}^{c}\rightarrow h_{\ell,ij}^{d,c}>m_\ell
\)
and
\(
\dot h_{\ell,ij}^{c}\rightarrow0
\).
Hence the adaptive-domain CBF constraint eventually ceases to require
positive enlargement. Since the auxiliary controller is the minimum
modification of
\(
v_{\ell,i}^{\mathrm{ref}}
=
-k_{s,\ell}s_{\ell,i}
\),
the selected input becomes negative for every
\(s_{\ell,i}>0\) and, in a neighborhood of \(s_{\ell,i}=0\),
coincides with the nominal recovery law. Therefore
\(
s_{\ell,i}\rightarrow0
\),
with exponential convergence once the recovery constraint becomes inactive.
\end{proof}

\begin{remark}
\label{rem:soft_clf_exactness}
The use of a linear--quadratic slack penalty additionally provides a local
exact-penalty interpretation. Consider the corresponding hard CLF-QP and let
\(\lambda_i^{h}\) denote the optimal multiplier associated with its CLF
constraint. Whenever the hard problem is feasible and
\(
\lambda_i^{h}<p_{1,i}
\),
the solution of the soft problem satisfies
\(
\delta_i^\star=0
\).
Hence, if the hard CLF-QP is feasible in a neighborhood of the desired set
and its multiplier remains below \(p_{1,i}\), the soft controller coincides
locally with the hard CLF controller.
\end{remark}

\begin{remark}
\label{rem:moving_leader_practical_tracking}
For a moving leader reference, the terms
\(
\veltwist_{1,\mathrm{ff}}
\)
and
\(
\dot{\veltwist}_{1,\mathrm{ff}}
\)
enter the comparison system as additional bounded inputs. Likewise, the
velocity of a moving parent enters \(\chi_i\). The same derivation therefore
gives a practical tracking result whose ultimate bound depends on the
reference motion in addition to the disturbances and CLF relaxation.
Exact asymptotic formation convergence without parent-velocity feedforward
requires an asymptotically stationary leader.
\end{remark}

\begin{remark}
\label{rem:global_convergence}
The above convergence result is local to a guarded region in which the hard
CLF condition is compatible with the bounded thruster authority. A global
or almost-everywhere convergence result would additionally require a
characterization of the critical points of the composite recentered-barrier
potential and of the global hard-CLF feasibility region. Such a
characterization is not required for the physical forward-invariance result
of Proposition~\ref{prop:adaptive_physical_invariance}.
\end{remark}
